Classical and quantum structuralism

In recent work, symmetric dagger-monoidal (SDM) categories have emerged as a convenient categorical formalization of quantum mechanics. The objects represent physical systems, the morphisms physical operations, whereas the tensors describe composite systems. Classical data turn out to correspond to Frobenius algebras with some additional properties. They express the distinguishing capabilities of classical data: in contrast with quantum data, classical data can be copied and deleted. The algebraic approach thus shifts the paradigm of "quantization" of a classical theory to "classicization" of a quantum theory. Remarkably, the simple SDM framework suffices not only for this conceptual shift, but even allows us to distinguish the deterministic classical operations (i.e. functions) from the nondeterministic classical operations (i.e. relations), and the probabilistic classical operations (stochastic maps). Moreover, a combination of some basic categorical constructions (due to Kleisli, resp. Grothendieck) with the categorical presentations of quantum states, provides a resource sensitive account of various quantum-classical interactions: of classical control of quantum data, of classical data arising from quantum measurements, as well as of the classical data processing in-between controls and measurements. A salient feature here is the graphical calculus for categorical quantum mechanics, which allows a purely diagrammatic representation of classical-quantum interaction.

==> MCPicts/Tele1b <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Sep 08 00:03:01 EDT 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.9" x-max="107.5" y-min="1.1" y-max="67.3" auto-bounding="true">
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(9,35.41);(9,58.78);(50.6,60.34);(50.6,35.41)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(34.1,24.8);(34.1,24.8);(34.1,36.68);(34.1,36.68)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50.6,25.13);(50.6,25.13);(50.6,37.01);(50.6,37.01)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(25.57,36.57);(25.57,43.13);(34.07,43.57);(34.07,36.57)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(34.17,24.81);(34.17,2.59);(75.9,1.1);(75.9,24.81)"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(50.7,25.6);(50.7,18.38);(59.5,17.9);(59.5,25.6)"
%	 />
%<ellipse closure= "open"
%	 p3= "(68.8,52.59)"
%	 stroke-style= "none"
%	 p1= "(66.8,50.52)"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 left-arrow= "head"
%	 p2= "(68.8,50.52)"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(68.44,51.57);(71.34,52.24);(71.34,53.55);(71.34,54.87)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.06,51.57);(64.3,52.24);(64.3,53.55);(64.3,54.87)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.8,47.97);(67.8,47.97);(67.8,51.32);(67.8,51.32)"
%	 />
%<multicurve fill-style= "solid"
%	 fill-color= "#cccccc"
%	 points= "(77.5,55.07);(77.5,55.07);(77.5,59.9);(77.5,59.9);(77.5,59.9);(72.34,59.9);
%	(72.34,59.9);(72.34,59.9);(69.77,55.07);(69.77,55.07);(69.77,55.07);(77.5,55.07);
%	(77.5,55.07)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(74.57,57.3)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\phi$
%</text>
%<multicurve fill-style= "solid"
%	 fill-color= "#cccccc"
%	 points= "(58.18,54.94);(58.18,54.94);(58.18,59.77);(58.18,59.77);(58.18,59.77);(63.32,59.77);
%	(63.32,59.77);(63.32,59.77);(65.88,54.94);(65.88,54.94);(65.88,54.94);(58.18,54.94);
%	(58.18,54.94)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(61.1,57.17)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\phi_*$
%</text>
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(59.4,25.18);(59.4,25.18);(59.3,38.78);(59.3,38.78)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(75.9,25);(75.9,25);(75.9,38.81);(75.9,38.81)"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(59.5,60);(59.5,60);(59.5,67.1);(59.5,67.1)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(76,60.2);(76,60.2);(76,67.3);(76,67.3)"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(9,1.8);(9,1.8);(9,35.45);(9,35.45)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(25.5,2.75);(25.5,2.75);(25.5,36.4);(25.5,36.4)"
%	 />
%<ellipse closure= "open"
%	 p3= "(68.83,45.86)"
%	 stroke-style= "none"
%	 p1= "(66.83,47.9)"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 left-arrow= "head"
%	 p2= "(68.83,47.9)"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(68.47,46.86);(71.37,46.2);(71.37,44.91);(71.37,43.61)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.09,46.86);(64.33,46.2);(64.33,44.91);(64.33,43.61)"
%	 />
%<multicurve fill-style= "solid"
%	 fill-color= "#cccccc"
%	 points= "(77.53,43.41);(77.53,43.41);(77.53,38.65);(77.53,38.65);(77.53,38.65);(72.37,38.65);
%	(72.37,38.65);(72.37,38.65);(69.8,43.41);(69.8,43.41);(69.8,43.41);(77.53,43.41);
%	(77.53,43.41)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(74.6,41.21)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\phi^\dagger$
%</text>
%<multicurve fill-style= "solid"
%	 fill-color= "#cccccc"
%	 points= "(58.21,43.54);(58.21,43.54);(58.21,38.78);(58.21,38.78);(58.21,38.78);(63.35,38.78);
%	(63.35,38.78);(63.35,38.78);(65.91,43.54);(65.91,43.54);(65.91,43.54);(58.21,43.54);
%	(58.21,43.54)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(61.13,41.34)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\phi^*$
%</text>
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(59.43,55.01);(59.43,55.01);(59.43,43.73);(59.43,43.73)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(75.93,54.7);(75.93,54.7);(75.93,43.41);(75.93,43.41)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(2.9,34.6)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%=
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(81.8,35)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%=
%</text>
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(91,10.4);(91,10.4);(91,56.6);(91,56.6)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(107.5,11.7);(107.5,11.7);(107.5,57.9);(107.5,57.9)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(107.5,67.3)
\psbezier{<-}(9,35.41)(9,58.78)(50.6,60.34)(50.6,35.41)
\psline(34.1,24.8)(34.1,36.68)
\psline(50.6,25.13)(50.6,37.01)
\psbezier{->}(25.57,36.57)(25.57,43.13)(34.07,43.57)(34.07,36.57)
\psbezier{->}(34.17,24.81)(34.17,2.59)(75.9,1.1)(75.9,24.81)
\psbezier{<-}(50.7,25.6)(50.7,18.38)(59.5,17.9)(59.5,25.6)
\rput{90}(67.8,51.56){\psellipse[linestyle=none,fillstyle=solid](0,0)(1.03,1)}
\psbezier(68.44,51.57)(71.34,52.24)(71.34,53.55)(71.34,54.87)
\psbezier(67.06,51.57)(64.3,52.24)(64.3,53.55)(64.3,54.87)
\psline(67.8,47.97)(67.8,51.32)
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](77.5,55.07)
(77.5,59.9)
(72.34,59.9)
(69.77,55.07)(77.5,55.07)
\rput(74.57,57.3){$\phi$}
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](58.18,54.94)
(58.18,59.77)
(63.32,59.77)
(65.88,54.94)(58.18,54.94)
\rput(61.1,57.17){$\phi_*$}
\psline{<-}(59.4,25.18)(59.3,38.78)
\psline{->}(75.9,25)(75.9,38.81)
\psline{<-}(59.5,60)(59.5,67.1)
\psline{->}(76,60.2)(76,67.3)
\psline{<-}(9,1.8)(9,35.45)
\psline{->}(25.5,2.75)(25.5,36.4)
\rput{90}(67.83,46.88){\psellipse[linestyle=none,fillstyle=solid](0,0)(1.02,-1)}
\psbezier(68.47,46.86)(71.37,46.2)(71.37,44.91)(71.37,43.61)
\psbezier(67.09,46.86)(64.33,46.2)(64.33,44.91)(64.33,43.61)
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](77.53,43.41)
(77.53,38.65)
(72.37,38.65)
(69.8,43.41)(77.53,43.41)
\rput(74.6,41.21){$\phi^\dagger$}
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](58.21,43.54)
(58.21,38.78)
(63.35,38.78)
(65.91,43.54)(58.21,43.54)
\rput(61.13,41.34){$\phi^*$}
\psline{<-}(59.43,55.01)(59.43,43.73)
\psline{->}(75.93,54.7)(75.93,43.41)
\rput(2.9,34.6){=}
\rput(81.8,35){=}
\psline{<-}(91,10.4)(91,56.6)
\psline{->}(107.5,11.7)(107.5,57.9)
\end{pspicture}


==> MCPicts/Tele2 <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Sep 08 02:15:13 EDT 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.9" x-max="71.4" y-min="1.09" y-max="67.29" auto-bounding="true">
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(2.9,35.4);(2.9,58.76);(44.87,60.33);(44.87,35.4)"
%	 />
%<ellipse closure= "open"
%	 p3= "(37.4,29.61)"
%	 stroke-style= "none"
%	 p1= "(35.4,27.54)"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 left-arrow= "head"
%	 p2= "(37.4,27.54)"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(37.04,28.59);(39.94,29.26);(39.94,30.57);(39.94,31.89)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35.66,28.59);(32.9,29.26);(32.9,30.57);(32.9,31.89)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.4,24.99);(36.4,24.99);(36.4,28.34);(36.4,28.34)"
%	 />
%<multicurve fill-style= "solid"
%	 fill-color= "#cccccc"
%	 points= "(46.1,32.09);(46.1,32.09);(46.1,36.92);(46.1,36.92);(46.1,36.92);(40.94,36.92);
%	(40.94,36.92);(40.94,36.92);(38.37,32.09);(38.37,32.09);(38.37,32.09);(46.1,32.09);
%	(46.1,32.09)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(43.17,34.32)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$U$
%</text>
%<multicurve fill-style= "solid"
%	 fill-color= "#cccccc"
%	 points= "(26.78,31.96);(26.78,31.96);(26.78,36.79);(26.78,36.79);(26.78,36.79);(31.92,36.79);
%	(31.92,36.79);(31.92,36.79);(34.48,31.96);(34.48,31.96);(34.48,31.96);(26.78,31.96);
%	(26.78,31.96)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(29.7,34.19)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$U_*$
%</text>
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(28,24.79);(28,24.79);(28,31.89);(28,31.89)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(44.5,24.99);(44.5,24.99);(44.5,32.09);(44.5,32.09)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(19.47,36.56);(19.47,43.12);(27.97,43.56);(27.97,36.56)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(28.07,25);(28.07,2.59);(69.8,1.09);(69.8,25)"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(44.6,25.59);(44.6,18.37);(53.4,17.89);(53.4,25.59)"
%	 />
%<ellipse closure= "open"
%	 p3= "(62.7,52.58)"
%	 stroke-style= "none"
%	 p1= "(60.7,50.51)"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 left-arrow= "head"
%	 p2= "(62.7,50.51)"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.34,51.56);(65.24,52.23);(65.24,53.54);(65.24,54.86)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60.96,51.56);(58.2,52.23);(58.2,53.54);(58.2,54.86)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(61.7,47.96);(61.7,47.96);(61.7,51.31);(61.7,51.31)"
%	 />
%<multicurve fill-style= "solid"
%	 fill-color= "#cccccc"
%	 points= "(71.4,55.06);(71.4,55.06);(71.4,59.89);(71.4,59.89);(71.4,59.89);(66.24,59.89);
%	(66.24,59.89);(66.24,59.89);(63.67,55.06);(63.67,55.06);(63.67,55.06);(71.4,55.06);
%	(71.4,55.06)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(68.47,57.29)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$U$
%</text>
%<multicurve fill-style= "solid"
%	 fill-color= "#cccccc"
%	 points= "(52.08,54.93);(52.08,54.93);(52.08,59.76);(52.08,59.76);(52.08,59.76);(57.22,59.76);
%	(57.22,59.76);(57.22,59.76);(59.78,54.93);(59.78,54.93);(59.78,54.93);(52.08,54.93);
%	(52.08,54.93)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,57.16)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$U_*$
%</text>
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(53.3,25.39);(53.3,25.39);(53.2,54.99);(53.2,54.99)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(69.8,24.99);(69.8,24.99);(69.8,55.06);(69.8,55.06)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.3,24.99);(36.3,12.49);(61.6,31.29);(61.6,48.09)"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(53.4,59.99);(53.4,59.99);(53.4,67.09);(53.4,67.09)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(69.9,60.19);(69.9,60.19);(69.9,67.29);(69.9,67.29)"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(2.9,1.79);(2.9,1.79);(2.9,35.45);(2.9,35.45)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(19.4,2.73);(19.4,2.73);(19.4,36.4);(19.4,36.4)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(71.4,67.29)
\psbezier{<-}(2.9,35.4)(2.9,58.76)(44.87,60.33)(44.87,35.4)
\rput{90}(36.4,28.58){\psellipse[linestyle=none,fillstyle=solid](0,0)(1.03,1)}
\psbezier(37.04,28.59)(39.94,29.26)(39.94,30.57)(39.94,31.89)
\psbezier(35.66,28.59)(32.9,29.26)(32.9,30.57)(32.9,31.89)
\psline(36.4,24.99)(36.4,28.34)
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](46.1,32.09)
(46.1,36.92)
(40.94,36.92)
(38.37,32.09)(46.1,32.09)
\rput(43.17,34.32){$U$}
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](26.78,31.96)
(26.78,36.79)
(31.92,36.79)
(34.48,31.96)(26.78,31.96)
\rput(29.7,34.19){$U_*$}
\psline{<-}(28,24.79)(28,31.89)
\psline{->}(44.5,24.99)(44.5,32.09)
\psbezier{->}(19.47,36.56)(19.47,43.12)(27.97,43.56)(27.97,36.56)
\psbezier{->}(28.07,25)(28.07,2.59)(69.8,1.09)(69.8,25)
\psbezier{<-}(44.6,25.59)(44.6,18.37)(53.4,17.89)(53.4,25.59)
\rput{90}(61.7,51.54){\psellipse[linestyle=none,fillstyle=solid](0,0)(1.03,1)}
\psbezier(62.34,51.56)(65.24,52.23)(65.24,53.54)(65.24,54.86)
\psbezier(60.96,51.56)(58.2,52.23)(58.2,53.54)(58.2,54.86)
\psline(61.7,47.96)(61.7,51.31)
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](71.4,55.06)
(71.4,59.89)
(66.24,59.89)
(63.67,55.06)(71.4,55.06)
\rput(68.47,57.29){$U$}
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](52.08,54.93)
(52.08,59.76)
(57.22,59.76)
(59.78,54.93)(52.08,54.93)
\rput(55,57.16){$U_*$}
\psline{<-}(53.3,25.39)(53.2,54.99)
\psline{->}(69.8,24.99)(69.8,55.06)
\psbezier(36.3,24.99)(36.3,12.49)(61.6,31.29)(61.6,48.09)
\psline{<-}(53.4,59.99)(53.4,67.09)
\psline{->}(69.9,60.19)(69.9,67.29)
\psline{<-}(2.9,1.79)(2.9,35.45)
\psline{->}(19.4,2.73)(19.4,36.4)
\end{pspicture}


==> MCPicts/Tele2b <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Sep 09 02:24:25 EDT 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.9" x-max="107.5" y-min="1.1" y-max="67.3" auto-bounding="true">
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(9,35.41);(9,58.78);(50.6,60.34);(50.6,35.41)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(34.1,24.8);(34.1,24.8);(34.1,36.68);(34.1,36.68)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50.6,25.13);(50.6,25.13);(50.6,37.01);(50.6,37.01)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25.57,36.57);(25.57,43.13);(34.07,43.57);(34.07,36.57)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(34.17,25);(34.17,2.6);(75.9,1.1);(75.9,25)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(50.7,25.6);(50.7,18.38);(59.5,17.9);(59.5,25.6)"
%	 />
%<ellipse closure= "open"
%	 p3= "(68.8,52.59)"
%	 stroke-style= "none"
%	 p1= "(66.8,50.52)"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 left-arrow= "head"
%	 p2= "(68.8,50.52)"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(68.44,51.57);(71.34,52.24);(71.34,53.55);(71.34,54.87)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.06,51.57);(64.3,52.24);(64.3,53.55);(64.3,54.87)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.8,47.97);(67.8,47.97);(67.8,51.32);(67.8,51.32)"
%	 />
%<multicurve fill-color= "#cccccc"
%	 fill-style= "solid"
%	 points= "(77.5,55.07);(77.5,55.07);(77.5,59.9);(77.5,59.9);(77.5,59.9);(72.34,59.9);
%	(72.34,59.9);(72.34,59.9);(69.77,55.07);(69.77,55.07);(69.77,55.07);(77.5,55.07);
%	(77.5,55.07)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(74.57,57.3)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$U$
%</text>
%<multicurve fill-color= "#cccccc"
%	 fill-style= "solid"
%	 points= "(58.18,54.94);(58.18,54.94);(58.18,59.77);(58.18,59.77);(58.18,59.77);(63.32,59.77);
%	(63.32,59.77);(63.32,59.77);(65.88,54.94);(65.88,54.94);(65.88,54.94);(58.18,54.94);
%	(58.18,54.94)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(61.1,57.17)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$U_*$
%</text>
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(59.4,25.18);(59.4,25.18);(59.3,38.78);(59.3,38.78)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75.9,25);(75.9,25);(75.9,38.81);(75.9,38.81)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(59.5,60);(59.5,60);(59.5,67.1);(59.5,67.1)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(76,60.2);(76,60.2);(76,67.3);(76,67.3)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(9,1.8);(9,1.8);(9,36.13);(9,36.13)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25.5,2.77);(25.5,2.77);(25.5,37.1);(25.5,37.1)"
%	 right-arrow= "head"
%	 />
%<ellipse closure= "open"
%	 p3= "(68.83,45.86)"
%	 stroke-style= "none"
%	 p1= "(66.83,47.9)"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 left-arrow= "head"
%	 p2= "(68.83,47.9)"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(68.47,46.86);(71.37,46.2);(71.37,44.91);(71.37,43.61)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.09,46.86);(64.33,46.2);(64.33,44.91);(64.33,43.61)"
%	 />
%<multicurve fill-color= "#cccccc"
%	 fill-style= "solid"
%	 points= "(77.53,43.41);(77.53,43.41);(77.53,38.65);(77.53,38.65);(77.53,38.65);(72.37,38.65);
%	(72.37,38.65);(72.37,38.65);(69.8,43.41);(69.8,43.41);(69.8,43.41);(77.53,43.41);
%	(77.53,43.41)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(74.6,41.21)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$U^\dagger$
%</text>
%<multicurve fill-color= "#cccccc"
%	 fill-style= "solid"
%	 points= "(58.21,43.54);(58.21,43.54);(58.21,38.78);(58.21,38.78);(58.21,38.78);(63.35,38.78);
%	(63.35,38.78);(63.35,38.78);(65.91,43.54);(65.91,43.54);(65.91,43.54);(58.21,43.54);
%	(58.21,43.54)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(61.13,41.34)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$U^*$
%</text>
%<multicurve fill-style= "none"
%	 points= "(59.43,55.01);(59.43,55.01);(59.43,43.73);(59.43,43.73)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(75.93,54.7);(75.93,54.7);(75.93,43.41);(75.93,43.41)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(2.9,34.6)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%=
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(81.8,35)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%=
%</text>
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(91,10.4);(91,10.4);(91,56.6);(91,56.6)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,11.7);(107.5,11.7);(107.5,57.9);(107.5,57.9)"
%	 right-arrow= "head"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(107.5,67.3)
\psbezier{<-}(9,35.41)(9,58.78)(50.6,60.34)(50.6,35.41)
\psline(34.1,24.8)(34.1,36.68)
\psline(50.6,25.13)(50.6,37.01)
\psbezier{->}(25.57,36.57)(25.57,43.13)(34.07,43.57)(34.07,36.57)
\psbezier{->}(34.17,25)(34.17,2.6)(75.9,1.1)(75.9,25)
\psbezier{<-}(50.7,25.6)(50.7,18.38)(59.5,17.9)(59.5,25.6)
\rput{90}(67.8,51.56){\psellipse[linestyle=none,fillstyle=solid](0,0)(1.03,1)}
\psbezier(68.44,51.57)(71.34,52.24)(71.34,53.55)(71.34,54.87)
\psbezier(67.06,51.57)(64.3,52.24)(64.3,53.55)(64.3,54.87)
\psline(67.8,47.97)(67.8,51.32)
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](77.5,55.07)
(77.5,59.9)
(72.34,59.9)
(69.77,55.07)(77.5,55.07)
\rput(74.57,57.3){$U$}
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](58.18,54.94)
(58.18,59.77)
(63.32,59.77)
(65.88,54.94)(58.18,54.94)
\rput(61.1,57.17){$U_*$}
\psline{<-}(59.4,25.18)(59.3,38.78)
\psline{->}(75.9,25)(75.9,38.81)
\psline{<-}(59.5,60)(59.5,67.1)
\psline{->}(76,60.2)(76,67.3)
\psline{<-}(9,1.8)(9,36.13)
\psline{->}(25.5,2.77)(25.5,37.1)
\rput{90}(67.83,46.88){\psellipse[linestyle=none,fillstyle=solid](0,0)(1.02,-1)}
\psbezier(68.47,46.86)(71.37,46.2)(71.37,44.91)(71.37,43.61)
\psbezier(67.09,46.86)(64.33,46.2)(64.33,44.91)(64.33,43.61)
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](77.53,43.41)
(77.53,38.65)
(72.37,38.65)
(69.8,43.41)(77.53,43.41)
\rput(74.6,41.21){$U^\dagger$}
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](58.21,43.54)
(58.21,38.78)
(63.35,38.78)
(65.91,43.54)(58.21,43.54)
\rput(61.13,41.34){$U^*$}
\psline{->}(59.43,55.01)(59.43,43.73)
\psline{<-}(75.93,54.7)(75.93,43.41)
\rput(2.9,34.6){=}
\rput(81.8,35){=}
\psline{<-}(91,10.4)(91,56.6)
\psline{->}(107.5,11.7)(107.5,57.9)
\end{pspicture}


==> MCPicts/Tele2c <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Sep 09 02:17:38 EDT 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.9" x-max="126.4" y-min="-11" y-max="85.13" auto-bounding="true">
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(2.9,40.9);(2.9,76.16);(69.3,78.53);(69.3,40.9)"
%	 />
%<ellipse closure= "open"
%	 p3= "(63.13,33.59)"
%	 stroke-style= "none"
%	 p1= "(61.13,31.52)"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 left-arrow= "head"
%	 p2= "(63.13,31.52)"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.77,32.57);(65.67,33.24);(65.67,34.55);(65.67,35.87)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(61.39,32.57);(58.63,33.24);(58.63,34.55);(58.63,35.87)"
%	 />
%<multicurve fill-color= "#cccccc"
%	 fill-style= "solid"
%	 points= "(71.83,36.07);(71.83,36.07);(71.83,40.9);(71.83,40.9);(71.83,40.9);(66.67,40.9);
%	(66.67,40.9);(66.67,40.9);(64.1,36.07);(64.1,36.07);(64.1,36.07);(71.83,36.07);
%	(71.83,36.07)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(68.9,38.3)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$U$
%</text>
%<multicurve fill-color= "#cccccc"
%	 fill-style= "solid"
%	 points= "(52.51,35.94);(52.51,35.94);(52.51,40.77);(52.51,40.77);(52.51,40.77);(57.65,40.77);
%	(57.65,40.77);(57.65,40.77);(60.21,35.94);(60.21,35.94);(60.21,35.94);(52.51,35.94);
%	(52.51,35.94)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(55.43,38.17)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$U_*$
%</text>
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(53.73,26.1);(53.73,26.1);(53.73,35.8);(53.73,35.8)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70.23,26.37);(70.23,26.37);(70.23,36.07);(70.23,36.07)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(19.3,40.7);(19.3,58.79);(53.7,60);(53.7,40.7)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(53.82,27.9);(53.82,-8.56);(124.8,-11);(124.8,27.9)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(70.2,27.5);(70.2,8.37);(108.4,7.1);(108.4,27.5)"
%	 />
%<ellipse closure= "open"
%	 p3= "(117.7,70.42)"
%	 stroke-style= "none"
%	 p1= "(115.7,68.35)"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 left-arrow= "head"
%	 p2= "(117.7,68.35)"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.34,69.4);(120.24,70.07);(120.24,71.38);(120.24,72.7)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115.96,69.4);(113.2,70.07);(113.2,71.38);(113.2,72.7)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(116.7,65.8);(116.7,65.8);(116.7,69.15);(116.7,69.15)"
%	 />
%<multicurve fill-color= "#cccccc"
%	 fill-style= "solid"
%	 points= "(126.4,72.9);(126.4,72.9);(126.4,77.73);(126.4,77.73);(126.4,77.73);(121.24,77.73);
%	(121.24,77.73);(121.24,77.73);(118.67,72.9);(118.67,72.9);(118.67,72.9);(126.4,72.9);
%	(126.4,72.9)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(123.47,75.13)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$U$
%</text>
%<multicurve fill-color= "#cccccc"
%	 fill-style= "solid"
%	 points= "(107.08,72.77);(107.08,72.77);(107.08,77.6);(107.08,77.6);(107.08,77.6);(112.22,77.6);
%	(112.22,77.6);(112.22,77.6);(114.78,72.77);(114.78,72.77);(114.78,72.77);(107.08,72.77);
%	(107.08,72.77)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,75)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$U_*$
%</text>
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(108.4,27.5);(108.4,27.5);(108.2,72.8);(108.2,72.8)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(124.8,27.9);(124.8,27.9);(124.8,72.9);(124.8,72.9)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.03,31.9);(62.03,20.4);(116.8,49.95);(116.8,65.4)"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(108.4,77.83);(108.4,77.83);(108.4,84.93);(108.4,84.93)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(124.9,78.03);(124.9,78.03);(124.9,85.13);(124.9,85.13)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(2.9,1.79);(2.9,1.79);(2.9,42);(2.9,42)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(19.4,2.73);(19.4,2.73);(19.3,40.7);(19.3,40.7)"
%	 right-arrow= "head"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(126.4,85.13)
\psbezier{<-}(2.9,40.9)(2.9,76.16)(69.3,78.53)(69.3,40.9)
\rput{90}(62.13,32.56){\psellipse[linestyle=none,fillstyle=solid](0,0)(1.03,1)}
\psbezier(62.77,32.57)(65.67,33.24)(65.67,34.55)(65.67,35.87)
\psbezier(61.39,32.57)(58.63,33.24)(58.63,34.55)(58.63,35.87)
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](71.83,36.07)
(71.83,40.9)
(66.67,40.9)
(64.1,36.07)(71.83,36.07)
\rput(68.9,38.3){$U$}
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](52.51,35.94)
(52.51,40.77)
(57.65,40.77)
(60.21,35.94)(52.51,35.94)
\rput(55.43,38.17){$U_*$}
\psline{<-}(53.73,26.1)(53.73,35.8)
\psline{->}(70.23,26.37)(70.23,36.07)
\psbezier{->}(19.3,40.7)(19.3,58.79)(53.7,60)(53.7,40.7)
\psbezier{->}(53.82,27.9)(53.82,-8.56)(124.8,-11)(124.8,27.9)
\psbezier{<-}(70.2,27.5)(70.2,8.37)(108.4,7.1)(108.4,27.5)
\rput{90}(116.7,69.38){\psellipse[linestyle=none,fillstyle=solid](0,0)(1.03,1)}
\psbezier(117.34,69.4)(120.24,70.07)(120.24,71.38)(120.24,72.7)
\psbezier(115.96,69.4)(113.2,70.07)(113.2,71.38)(113.2,72.7)
\psline(116.7,65.8)(116.7,69.15)
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](126.4,72.9)
(126.4,77.73)
(121.24,77.73)
(118.67,72.9)(126.4,72.9)
\rput(123.47,75.13){$U$}
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](107.08,72.77)
(107.08,77.6)
(112.22,77.6)
(114.78,72.77)(107.08,72.77)
\rput(110,75){$U_*$}
\psline{<-}(108.4,27.5)(108.2,72.8)
\psline{->}(124.8,27.9)(124.8,72.9)
\psbezier(62.03,31.9)(62.03,20.4)(116.8,49.95)(116.8,65.4)
\psline{<-}(108.4,77.83)(108.4,84.93)
\psline{->}(124.9,78.03)(124.9,85.13)
\psline{<-}(2.9,1.79)(2.9,42)
\psline{->}(19.4,2.73)(19.3,40.7)
\end{pspicture}


==> MCPicts/Tele2d <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Sep 09 02:46:02 EDT 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.9" x-max="129" y-min="-5.4" y-max="88.7" auto-bounding="true">
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(9,40.4);(9,71.8);(65.7,73.9);(65.7,40.4)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(49.6,25.4);(49.6,25.4);(49.6,41.16);(49.6,41.16)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65.6,25.84);(65.6,25.84);(65.6,41.6);(65.6,41.6)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25.4,40.4);(25.4,54.36);(49.6,55.3);(49.6,40.4)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(49.6,26.5);(49.6,-3.4);(97.33,-5.4);(97.33,26.5)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(65.77,26.1);(65.77,14.38);(80.7,13.6);(80.7,26.1)"
%	 />
%<ellipse closure= "open"
%	 p3= "(90.27,73.99)"
%	 stroke-style= "none"
%	 p1= "(88.27,71.92)"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 left-arrow= "head"
%	 p2= "(90.27,71.92)"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(89.91,72.97);(92.81,73.64);(92.81,74.95);(92.81,76.27)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(88.53,72.97);(85.77,73.64);(85.77,74.95);(85.77,76.27)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(89.27,69.37);(89.27,69.37);(89.27,72.72);(89.27,72.72)"
%	 />
%<multicurve fill-color= "#cccccc"
%	 fill-style= "solid"
%	 points= "(98.97,76.47);(98.97,76.47);(98.97,81.3);(98.97,81.3);(98.97,81.3);(93.81,81.3);
%	(93.81,81.3);(93.81,81.3);(91.24,76.47);(91.24,76.47);(91.24,76.47);(98.97,76.47);
%	(98.97,76.47)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(96.04,78.7)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$U$
%</text>
%<multicurve fill-color= "#cccccc"
%	 fill-style= "solid"
%	 points= "(79.65,76.34);(79.65,76.34);(79.65,81.17);(79.65,81.17);(79.65,81.17);(84.79,81.17);
%	(84.79,81.17);(84.79,81.17);(87.35,76.34);(87.35,76.34);(87.35,76.34);(79.65,76.34);
%	(79.65,76.34)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(82.57,78.57)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$U_*$
%</text>
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(80.87,26.15);(80.87,26.15);(80.77,60.14);(80.77,60.14)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(97.37,25.7);(97.37,25.7);(97.37,60.21);(97.37,60.21)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(80.97,81.4);(80.97,81.4);(80.97,88.5);(80.97,88.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(97.47,81.6);(97.47,81.6);(97.47,88.7);(97.47,88.7)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(9,1.8);(9,1.8);(9,41.38);(9,41.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25.5,2.92);(25.5,2.92);(25.5,42.5);(25.5,42.5)"
%	 right-arrow= "head"
%	 />
%<ellipse closure= "open"
%	 p3= "(90.3,67.26)"
%	 stroke-style= "none"
%	 p1= "(88.3,69.3)"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 left-arrow= "head"
%	 p2= "(90.3,69.3)"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(89.94,68.26);(92.84,67.6);(92.84,66.31);(92.84,65.01)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(88.56,68.26);(85.8,67.6);(85.8,66.31);(85.8,65.01)"
%	 />
%<multicurve fill-color= "#cccccc"
%	 fill-style= "solid"
%	 points= "(99,64.81);(99,64.81);(99,60.05);(99,60.05);(99,60.05);(93.84,60.05);
%	(93.84,60.05);(93.84,60.05);(91.27,64.81);(91.27,64.81);(91.27,64.81);(99,64.81);
%	(99,64.81)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(96.07,62.61)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$U^\dagger$
%</text>
%<multicurve fill-color= "#cccccc"
%	 fill-style= "solid"
%	 points= "(79.68,64.94);(79.68,64.94);(79.68,60.18);(79.68,60.18);(79.68,60.18);(84.82,60.18);
%	(84.82,60.18);(84.82,60.18);(87.38,64.94);(87.38,64.94);(87.38,64.94);(79.68,64.94);
%	(79.68,64.94)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(82.6,62.74)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$U^*$
%</text>
%<multicurve fill-style= "none"
%	 points= "(80.9,76.41);(80.9,76.41);(80.9,65.13);(80.9,65.13)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(97.4,76.1);(97.4,76.1);(97.4,64.81);(97.4,64.81)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(2.9,34.6)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%=
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(105,35)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%=
%</text>
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(115,10.4);(115,10.4);(115,56.6);(115,56.6)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(129,10);(129,10);(129,56.2);(129,56.2)"
%	 right-arrow= "head"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(129,88.7)
\psbezier{<-}(9,40.4)(9,71.8)(65.7,73.9)(65.7,40.4)
\psline(49.6,25.4)(49.6,41.16)
\psline(65.6,25.84)(65.6,41.6)
\psbezier{->}(25.4,40.4)(25.4,54.36)(49.6,55.3)(49.6,40.4)
\psbezier{->}(49.6,26.5)(49.6,-3.4)(97.33,-5.4)(97.33,26.5)
\psbezier{<-}(65.77,26.1)(65.77,14.38)(80.7,13.6)(80.7,26.1)
\rput{90}(89.27,72.96){\psellipse[linestyle=none,fillstyle=solid](0,0)(1.03,1)}
\psbezier(89.91,72.97)(92.81,73.64)(92.81,74.95)(92.81,76.27)
\psbezier(88.53,72.97)(85.77,73.64)(85.77,74.95)(85.77,76.27)
\psline(89.27,69.37)(89.27,72.72)
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](98.97,76.47)
(98.97,81.3)
(93.81,81.3)
(91.24,76.47)(98.97,76.47)
\rput(96.04,78.7){$U$}
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](79.65,76.34)
(79.65,81.17)
(84.79,81.17)
(87.35,76.34)(79.65,76.34)
\rput(82.57,78.57){$U_*$}
\psline{<-}(80.87,26.15)(80.77,60.14)
\psline{->}(97.37,25.7)(97.37,60.21)
\psline{<-}(80.97,81.4)(80.97,88.5)
\psline{->}(97.47,81.6)(97.47,88.7)
\psline{<-}(9,1.8)(9,41.38)
\psline{->}(25.5,2.92)(25.5,42.5)
\rput{90}(89.3,68.28){\psellipse[linestyle=none,fillstyle=solid](0,0)(1.02,-1)}
\psbezier(89.94,68.26)(92.84,67.6)(92.84,66.31)(92.84,65.01)
\psbezier(88.56,68.26)(85.8,67.6)(85.8,66.31)(85.8,65.01)
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](99,64.81)
(99,60.05)
(93.84,60.05)
(91.27,64.81)(99,64.81)
\rput(96.07,62.61){$U^\dagger$}
\newrgbcolor{userFillColour}{0.8 0.8 0.8}
\psline[fillcolor=userFillColour,fillstyle=solid](79.68,64.94)
(79.68,60.18)
(84.82,60.18)
(87.38,64.94)(79.68,64.94)
\rput(82.6,62.74){$U^*$}
\psline{->}(80.9,76.41)(80.9,65.13)
\psline{<-}(97.4,76.1)(97.4,64.81)
\rput(2.9,34.6){=}
\rput(105,35){=}
\psline{<-}(115,10.4)(115,56.6)
\psline{->}(129,10)(129,56.2)
\end{pspicture}


==> MCPicts/ids.tex <==
%Created by jPicEdt 1.x
%PsTricks format (pstricks.sty needed)
%Sat Feb 24 15:16:18 EST 2007
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\begin{pspicture}(0,0)(60.80,19.80)
\psline[linewidth=0.30,linecolor=black]{->}(5.90,0.00)(5.90,19.80)
\psline[linewidth=0.30,linecolor=black]{<-}(55.90,0.00)(55.90,19.80)
\rput(11.00,4.00){$A$}
\rput(60.80,4.10){$A$}
\end{pspicture}

